Generation-driven Contrastive Self-training for Zero-shot Text Classification with Instruction-following LLM

The remarkable performance of large language models (LLMs) in zero-shot language understanding has garnered significant attention. However, employing LLMs for large-scale inference or domain-specific fine-tuning requires immense computational resources due to their substantial model size. To overcome these limitations, we introduce a novel method, namely GenCo, which leverages the strong generative power of LLMs to assist in training a smaller and more adaptable language model. In our method, an LLM plays an important role in the self-training loop of a smaller model in two important ways. Firstly, the LLM is used to augment each input instance with a variety of possible continuations, enriching its semantic context for better understanding. Secondly, it helps crafting additional high-quality training pairs, by rewriting input texts conditioned on predicted labels. This ensures the generated texts are highly relevant to the predicted labels, alleviating the prediction error during pseudo-labeling, while reducing the dependency on large volumes of unlabeled text. In our experiments, GenCo outperforms previous state-of-the-art methods when only limited ($<5\%$ of original) in-domain text data is available. Notably, our approach surpasses the performance of Alpaca-7B with human prompts, highlighting the potential of leveraging LLM for self-training.

==> tex/998.method_copy.tex <==


%Separate the proposed method into two sections, 

% (1)Briefly explain the novelty of using instr-gpt for data augmentation. (1).1 How we use instr-gpt for augmentation: for inference, for creating positive pairs between non-augmented/augmented texts,  for creating hard negative samples, and introduce some notation of augmentation here (1).2 using GPT to create more correct texts

% (2)self-training for contrastive learning: first give an overview of the method using Figure 1, then (2).1 introduce zero-shot classification as sentence alignment and how we perform inference and mention we can use instr-GPT in the next section for augmentation (2).2 contrastive learning loss -> (a)contrastive loss (b) (2).3 how we conduct self-training using contrastive loss



\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/fig_general_aug.pdf}
    \caption{Input Text Augmentation with intruction-tuned GPT: The input text and an instruction are fed into the GPT model to generate multiple pieces of elaborated texts, each of which is concatenated to the original input to obtain an augmented text. The embeddings of the augmented texts are then averaged to obtain a merged embedding, which is used for label prediction in the self-training process. }
    \label{fig:general_aug_illustration}
\end{figure*}


\section{Preliminary: Zero-shot Text Classification as Sentence Alignment}
\label{sec:method}
%The task of zero-shot text classification involves predicting the most relevant labels for a given document without requiring any labeled training data.
Given a set of $N$ unlabeled documents $X=\{x_1,x_2,\cdots,x_N \}$ and a set of $L$ category descriptions $C=\{c_1,c_2,\cdots,c_L \}$, the goal is to learn a scoring function $g(x,c_i)$ that takes document $x$ and label description $c_i$ as input and produces a similarity score as the measure of how well the document and the label match to each other. 
%In the rest of the paper, we assume each input text as a sentence for convenience, which can be easily generalized to a multi-sentence passage or document without jeopardizing the key concepts.

In the zero-shot setting, text classification can be formulated as a sentence alignment problem, where both the both the input sentence and the label descriptions are encoded using a pre-trained sentence encoder like SimCSE~\cite{gao2021simcse}. The similarity scores between the sentence and labels embeddings are used to predict related labels. The performance can be further improved by converting a short label description into a full sentence via prompts~\cite{wang2023pesco, hong2022tess}. For example, the label ``sports" can be converted to ``This is an article about sports."
%Since this approach relies on the semantic matching between textual instances and label descriptions rather than the availability of labeled training data
%However, as label descriptions are often just a few words instead of long sentences, they may not provide enough context for a pre-trained encoder to grasp the semantic meaning of the labels. To address this issue, prompt-based approaches \cite{schick2020exploiting} convert label names into natural language sentences, namely \textit{label prompts}. For example, the label ``sports" can be converted to ``This is an article about sports." 
Following this, we denote by $p_i$ as the label prompt for a label description $c_i$, the scoring function can be implemented as:
\begin{equation}
    g(x, c_i)=\operatorname{sim}\left(f_\theta(x), f_\theta(p_i) \right)
\end{equation}
where $f_\theta(\cdot)$ is the sentence encoder parameterized by $\theta$ and $\mathrm{sim}(\cdot,\cdot)$ is a similarity function such as dot product or cosine similarity.

Given a input text at inference time, the predicted  label is the one with the highest similarity score:
\begin{equation}
\hat{y}=\argmax_j g\left(x, c_j\right) \label{eq:inference}
\end{equation}

\section{Our Method: \ourmodel}
We first propose and analyze a contrastive self-training objective, and the present our generative approach to enhance the self-training loop.

\subsection{Contrastive Self-Training Objective}
\label{subsec:self-training}
Self-training is an algorithm to enhance the generalization capability of models by learning from its own predictions~\cite{meng2020text,schick2021self,wang2023pesco}. 
%Specifically, it follows an iterative process where a pre-trained model is used to classify unlabeled data, and the newly classified data with high confidence is then used to further train the model. 
Since the predicted labels can be erroneous, studies have shown that soft labeling~\cite{xie2016unsupervised,meng2020text} or label smoothing~\cite{muller2019does} can prevent the model from becoming overly confident. In this work, we propose a loss function with soft labeling that connects supervised contrastive learning and entropy regularization~\cite{grandvalet2004semi}. Our analysis aims to reveal how self-training can improve the zero-shot generalization by maximizing the decision boundaries of ambiguous classes.

%We denote $f_\theta(x)$ as our sentence encoder model. 
Given a input text $x$, the predicted distribution of the label space is:
\begin{equation}
    P(\hat{y}_i | x ;\theta) =  \frac{\exp(\operatorname{sim}(f_\theta(x), f_\theta(p_i)))}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x), f_\theta(p_c)))} 
\end{equation}
Here, $p_i$ is a label prompt for label $c_i$. We define the target distribution as:
\begin{equation}
    Q(\hat{y}_i | x ;\theta) =   \frac{\exp(\operatorname{sim}(f_\theta(x), f_\theta(p_i))/\tau)}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x), f_\theta(p_c))/\tau)} \label{eq:soft-label}
\end{equation}
where $\tau \leq 1$ is the temperature. A lower temperature implies a sharper distribution and thus greater confidence in the predicted label. We drop the notation of $\theta$ for convenience.

Our proposed text to label ($t2l$) contrastive loss is defined as:
\begin{equation}
    \mathcal{L}_{t2l} = -\sum_{i=1}^{N} \sum_{j=1}^{L} Q(\hat{y}_j|x_i)\log P(\hat{y}_j|x_i) \label{eq:loss}
\end{equation}
When $\tau \rightarrow 0$, $Q(\hat{y} | x)$ becomes categorical distribution and the loss reduces to a supervised contrastive learning loss with pseudo label $\hat{y}$ as the target:
\begin{equation}
    \mathcal{L}_{t2l}^{\tau \rightarrow 0} = -\sum_{i=1}^{N} \log P(\hat{y}|x_i)
\end{equation}
It encourages the model to predict label $\hat{y}$ given $x$ with more confident. 
On the other hand, when $\tau = 1$, the loss reduces to a minimization of conditional entropy function $H$:
\begin{align}
    &\mathcal{L}_{t2l}^{\tau = 1} = H\left(C \mid X \right) \\
    &= - \sum_{i=1}^N\sum_{j=1}^L P(\hat{y}_j|x_i)\log P(\hat{y}_j|x_i)
\end{align}
We show a theorem such that minimizing the loss function \eqref{eq:loss} can achieve similar effects Entropy Regularization~\cite{grandvalet2006entropy,grandvalet2004semi}, which is a means to enforce the cluster assumption such that the decision boundary should lie in low-density regions to improve generalization performance~\cite{chapelle2005semi}. 
\begin{theorem}
\label{theorem:paper}
Consider a binary classification problem with linearly separable labeled examples. When $0<\tau<1$, optimizing \eqref{eq:loss} with gradient descend will enforce the larger margin between classes and achieves max margin classifier under certain constraint. 
\end{theorem}
We place our formal theorems and proofs in Appendix \secref{sec:proofs}. Theorem \ref{theorem:1}  suggests that self-training is an in domain fine-tuning that maximizes class separation, which serves as an explanation why training on pseudo-labels can enhance performance even if no extra labeling information is provided.
In our experiment, we show empirically that self-training of smaller model can outperform Alpaca-7B prediction. We set $\tau = 0.1$ to balance supervised classification and low density separation between classes. 


%While self-learning was effective in improving the performance of our model, it is not without its limitations. One potential issue is overfitting to the pseudo label, which is prone to error. Additionally, self-learning requires a large amount of unlabeled data, which may not always be available.
%In the following section, we propose conditional augmentation methods with generative model in the training loop to make self-learning more robust. 

% \subsection{GenCo}
% \label{subsec:conditional augment}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/fig_cond_aug.pdf}
    \caption{Augmented Text Generation Conditioned on Pseudo Labels: When a pseudo label is incorrect, it can mislead the training process and decrease classification performance. We generate augmented text conditioned on the pseudo label, aiming to make the generated text closer to the majority members in the category of the pseudo label. This approach aims to improve the quality of the generated instances for self-training. }
    \label{fig:conditional_aug_illustration}
\end{figure*}

While self-training can potentially improve model generalization, the limitations are obvious: 1) pseudo labels are prone to error and can negatively affect model training. 2) self-learning requires a significant load of unlabeled data, which may not always be available. Next, we introduce generation-driven approaches to improve self-training with an instruction-tuned GPT.

\subsection{Input Text Augmentation}
\label{subsec:input augment}
In this section, we propose a way to enrich the semantic information of the input text with multiple GPT-generated pieces of texts, as shown in \figref{fig:general_aug_illustration}. When the input text is relatively short, such as consisting of only one or a few sentences, the information may not be sufficient for alignment-based matching to relevant labels. A remedy is to ask GPT model to elaborate the input and generate multiple pieces of extended texts. Specifically, we use a simple human instruction, "Elaborate the text with a few sentences," to guide the instruction-tuned GPT model, such as Alpaca-7B~\cite{alpaca}, in generating probable expansions and continuations of the text. Our system treats the concatenation of the input text and each GPT-generated piece as one augmentation, and then takes the average of the embeddings of multiple augmentations as the merged embedding of the augmented input. 
%Intuitively, such an augmentation should enhance the semantic matching among input text and relevant labels if the meaning of the input is underrepresented (too short) and if the generative model is highly effective in generating relevant pieces for the given input.  The first assumption is often true in realist textual data, and the second condition is well-met by large pre-trained GPT models.  
%Formally, the input text $x \sim P(x)$ can be viewed as randomly sampled from an underlying distribution, and 

Given the original input $x$, the augmented texts are sampled from the conditional probability distribution induced by the GPT model, denoted as $x^{\text{aug}} \sim P_g(\cdot | x)$. $x^{\text{aug}}$ is used in two places in self-training:

First, we use the augmented text for more robust pseudo-label prediction. We enhance the input embedding by:
\begin{equation}
\frac{1}{K}\sum_{i=1}^K f_\theta(x \oplus x_i^{\text{aug}}),
\end{equation}
where $\oplus$ is the concatenation operator for text and $x_i^{\text{aug}}$ is the $i$-th sample from $P_g(\cdot | x)$. The mean of the embedding gives an ensemble of GPT induced features. 

Secondly, we propose a contrastive loss between input text and generated text for optimization. Let $\mathit{I}$ be a training batch and $A(i)$ 
be the set of augmented texts with the same pseudo-label as input $x_i$. Therefore, $x$ and $x^{\text{aug}}$ ($\in A(i)$) should be similar in the embedding space:
\begin{equation} 
\begin{split}
     &\mathcal{L}_{t2g}=\sum_{i \in \mathit{I}} \frac{ -1}{|A(i)|} \\ 
     &\sum_{x^{\text{aug}} \in A(i)}\log{\frac{\exp({sim(f_{\theta}(x_i),f_{\theta}(x^{\text{aug}}) )})}{\sum_{j \in \mathit{I}}\exp(sim(f_{\theta}(x_i),f_{\theta}(x_j) ))}}.
\end{split} \label{eq:t2g}
\end{equation}


%If GPT is available at test time, we can use this method for inference as well.

\subsection{Augmentation Conditioned on Prediction}
% The success of the algorithm relies on two key factors: 1) the availability of diversified instances for self-training, and 2) the accurate assignment of pseudo label for the unlabeled text. However, it is difficult to satisfy the two conditions at the same time. On the one hand, if self-training is applied to only the highly confident instances, the amount of training instance is too limited to the effectiveness of the algorithm. On the other hand, if we apply the algorithm to large amount of unlabeled data with lower confidence, the inaccurate pseudo labeling can lead to negative transfer and hurt the performance of the classifier.
%The loss function of \eqref{eq:loss} can effectively enhance the separability of class instances by enforcing the decision boundary to lie in low density regions of the embedding space. In each self-training iteration, when the sampled instances are labeled with relatively lower confidence, which lie near the decision boundary, 
%The contrastive loss in \eqref{eq:loss} pushes the instance embedding closer to the pseudo label prompt embedding. However, 
Self-training can lead to an undesirable bias in the classifier when instances are mislabeled. To address this issue, we propose an approach to generate high quality pseudo-labeled data pairs for self-training, as shown in \figref{fig:conditional_aug_illustration}.
%Specifically, we use GPT to generate training instances conditioned on the pseudo-labels, . 
For example, if a "business" article discussing the retirement of Starbucks' president is misclassified as "sports", optimizing the model with this mislabeled training instance will make the decision boundaries of business articles less separable from sport articles. To alleviate such an undesirable effect, we use GPT to augment the input text conditioned on the sport category by constructing instructions such as "Discuss the sports aspects of the article". As a result, we
obtain a generated text that looks like typical ones in the sport category and optimize on the new one instead of the original one which lies on the wrong side of decision boundary between "sports" and "business". In other words, by generating texts conditioned on pseudo labels, we synthesize training pairs with better separation of class labels in the embedding space, and thus alleviating the issue of mislabeling encountered during self-training.  

Let $x^\text{cond} \sim P_g(\cdot | x, \hat{y})$ be the conditionally augmented text, the modified \eqref{eq:loss} is:
% To alleviate the problem of erroneous label assignment, we use the conditional augmented text ($x^{\text{c\_aug}} \sim P_g(\cdot | x, \hat{y})$) and the pseudo label prompt as positive pairs. 
\begin{equation}
    \mathcal{L}_{g2l} = -\sum_{i=1}^{N} \sum_{j=1}^{L} Q(\hat{y}_j|x_i^{\text{cond}})\log P(\hat{y}_j|x_i^{\text{cond}})
    \label{eq:g2l}
\end{equation}


%propose an approach called \textit{instruction-based conditional generation} to generate augmented text conditioned on the pseudo label. In this approach, we incorporate the predicted label information into the instructions provided to the model. For instance, we can use the instruction ``Discuss the sports aspects of the article" to guide the model in generating text that is more relevant to the sports category.

%By providing these instructions, we ensure the generated text is more accurate and diverse, which can alleviate the problem of overfitting to mislabeled data during self-training. In the following, w
%Additionally, we propose two loss functions to enhance the self-training algorithm with the augmented text as follows.

\begin{algorithm*}[ht!]
  \caption{Self-training with GPT model assisted in the loop}
  \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, instruction-tuned GPT model $g(\cdot)$.\\
  \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
  \textbf{Input augmentation}: For each observed text, generate $K$ samples of augmented text from $P_g(\cdot | x)$.\\
  \For {$t: 1 \rightarrow T$ self-training iterations}
  {
    Use $f_{\theta}(\cdot)$ to generate pseudo-labels $\hat{y}$ (eq.\ref{eq:inference}) and soft-target $Q$ (eq.\ref{eq:soft-label}) for texts with input augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ according to prediction confidence\;
    \For {each training sample $(x, \hat{y})$}
    {
        \eIf{key $(x, \hat{y}) \in \operatorname{GenDict}$}
        {
            Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
        }
        {
            Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}\;
            Add generated texts to $\operatorname{GenDict}$\Comment{Cached generated text}\;
        }
    }
    Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$.
  }
 % \textbf{Return:} $f_{\theta}(\cdot)$
\label{alg:self-train}
\end{algorithm*}

% \subsubsection{Contrastive Learning for Conditionally Augmented Text and Label Prompt} To alleviate the problem of erroneous label assignment, we use the conditional augmented text ($x^{\text{c\_aug}} \sim P_g(\cdot | x, \hat{y})$) and the pseudo label prompt as positive pairs. 
% \begin{equation}
%     \mathcal{L}_{g2l} = -\sum_{i=1}^{N} \sum_{j=1}^{L} Q(\hat{y}_j|x_i^{\text{c\_aug}})\log P(\hat{y}_j|x_i^{\text{c\_aug}})
%     %-\log P(\hat{y}_i | x ;\theta) = -\log \frac{\exp(\operatorname{sim}(f_\theta(x_\text{aug}), f_\theta(p_i)))}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x_\text{aug}), f_\theta(p_c)))} 
%     \label{eq:g2l}
% \end{equation}

%\subsubsection{Contrastive Learning for Observed Text and Augmented Text} 
%The essence of contrastive learning is to compare different views of data for representation learning~\cite{chen2020simple,he2020momentum}. 

\subsection{Algorithm for Self-training}
We apply self-training in a iterative way as shown in \Algref{alg:self-train} with generative model assisting in the  loop. During training, we found that a balanced sampling that keeps the same number ($S_t$ for iteration $t$) of training for each category is important for the stability of self-training. Additionally, we use a dictionary to cache the conditional generated text to avoid repeated generation. 


%Overall, our proposed approach provides a flexible and effective way to generate augmented text that can improve the performance of smaller classifiers. By conditioning the GPT model on the predicted label, we can generate additional text that is specifically tailored to the characteristics of each class, which can help the classifier better distinguish between different classes. Our approach can also help address the issues of limited diversity and inaccurate pseudo labeling in self-training, by providing more diverse and accurate instances for self-training.

%suffers from wrong labels. We condition the GPT model on the current predicted label to generate additional augmented text that is tailored to the specific label. We explore the following methods for conditional generation of augmented text $x^\prime \sim P_g(\cdot| x, \hat{y})$.

%In label-based conditional generation, we directly incorporate the predicted label $\hat{y}$ into the generation process. Specifically, we condition the GPT model on both the original text $x$ and the predicted label $\hat{y}$ to generate augmented text $x^\prime$. This approach allows the model to better capture the specific characteristics and features of each class.



% \subsubsection{Prompt-based Conditional Generation} To let the model condition on label, we append a short prompt after the original text $x$, such as ``In this sports article,". 

% \subsubsection{Instruction-based Conditional Generation}
% Previous work have shown that language models have the ability to take instructions~\cite{brown2020language,ouyang2022training}. We construction natural language instructions for the language model to generate augmented text, such as "continue writing the above paragraph from the perspective of sports".

% The GPT model can then generate additional text based on this prompt. By conditioning the model on the predicted label, we can generate augmented text that is specifically tailored to the characteristics of the sports class.

% Overall, these three methods provide flexible and effective ways to generate augmented text that can improve the performance of smaller classifiers. By conditioning the GPT model on the predicted label, we can generate additional text that is specifically tailored to the characteristics of each class, which can help the classifier better distinguish between different classes.

%\subsubsection{Generation with Word Mask} 
% Another approach for conditional generation is to give the model higher probability on topic sensitive words. In this paper, we propose a method based on topical words:
% \begin{align}
%     \delta &= p(w|y) - p(w|x) \\
%     p(w|x,y) &\propto \alpha(\delta)p(w|x)
% \end{align}
    
%~\cite{schick2021self} use 

% \begin{algorithm}
% $i\gets 10$\;
% \eIf{$i\geq 5$}
% {
%     $i\gets i-1$\;
% }{
%     \If{$i\leq 3$}
%     {
%         $i\gets i+2$\;
%     }
% }
% \end{algorithm}
  
% \begin{algorithm}
%   \caption{Self-training with GPT model in the training loop}
%   \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, pre-trained GPT model $g(\cdot)$.\\
%   \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
%   \begin{algorithmic}[1]
%   %\Procedure{Self-train}{$n$}
%   \State \textbf{General purpose augmentation}: For each observed text, sample $K$ views  from $P_g(\cdot | x)$ as general augmented data.
%   \For {$t: 1 \rightarrow T$ self-training iterations}:
%     \parState {Use $f_{\theta}(\cdot)$ to generate soft pseudo-labels $\hat{y}$ with eq.(\ref{eq:inference}) for unlabeled texts with general purpose augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ for each label according to confidence. }
%     \For {each training sample $(x, \hat{y})$}, 
%     \If{$(x, \hat{y}) \in \operatorname{GenDict}$}
%         \State Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
%     \Else
%         \State Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}
%         \State Add generated texts to $\operatorname{GenDict}$\Comment{cached generated text}
%     \EndIf
%     \EndFor
%     \parState {Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$ in eq~\ref{eq:loss}.}
%   \EndFor
    
%   \State \textbf{Return:} $f_{\theta}(\cdot)$
%   %\textbf{Final model:} Use $f_{\theta}(\cdot)$ to label the full unlabeled set, then uses the pseudo-labels to learn a new model as final model.
%   %\EndProcedure
%  \end{algorithmic}
%  \label{alg:self-train}
% \end{algorithm}

% \begin{algorithm}[ht!]
%   \caption{Self-training with GPT model in the training loop}
%   \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, pre-trained GPT model $g(\cdot)$.\\
%   \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
%   \textbf{General purpose augmentation}: For each observed text, sample $K$ views  from $P_g(\cdot | x)$ as general augmented data.\\
%   \For {$t: 1 \rightarrow T$ self-training iterations}
%   {
%     Use $f_{\theta}(\cdot)$ to generate soft pseudo-labels $\hat{y}$ with eq.(\ref{eq:inference}) for unlabeled texts with general purpose augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ for each label according to confidence\;
%     \For {each training sample $(x, \hat{y})$}
%     {
%         \eIf{$(x, \hat{y}) \in \operatorname{GenDict}$}
%         {
%             Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
%         }
%         {
%             Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}\;
%             Add generated texts to $\operatorname{GenDict}$\Comment{Cached generated text}\;
%         }
%     }
%     Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$ in eq~\ref{eq:loss}.
%   }
%  % \textbf{Return:} $f_{\theta}(\cdot)$
% \label{alg:self-train}
% \end{algorithm}

==> tex/999.tmp.tex <==
\section{Our Method: \ourmodel}

%Separate the proposed method into two sections, 

% (1)Briefly explain the novelty of using instr-gpt for data augmentation. (1).1 How we use instr-gpt for augmentation: for inference, for creating positive pairs between non-augmented/augmented texts,  for creating hard negative samples, and introduce some notation of augmentation here (1).2 using GPT to create more correct texts

% (2)self-training for contrastive learning: first give an overview of the method using Figure 1, then (2).1 introduce zero-shot classification as sentence alignment and how we perform inference and mention we can use instr-GPT in the next section for augmentation (2).2 contrastive learning loss -> (a)contrastive loss (b) (2).3 how we conduct self-training using contrastive loss


\label{sec:method}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/fig_general_aug.pdf}
    \caption{Input Text Augmentation using GPT Models: The input text and an instruction are fed into the GPT model to generate multiple pieces of elaborated texts, each of which is concatenated to the original input to obtain an augmented text. The embeddings of the augmented texts are then averaged to obtain a merged embedding, which is used for label prediction in the self-training process. }
    \label{fig:general_aug_illustration}
\end{figure*}

We first introduce the sentence encoder classifier as our basic design choice, and then focus on the novel components in our framework in the follow-up sections.

\subsection{Zero-shot Text Classification as Sentence Alignment}
%The task of zero-shot text classification involves predicting the most relevant labels for a given document without requiring any labeled training data. 
Given a set of $N$ unlabeled documents $X=\{x_1,x_2,\cdots,x_N \}$ and a set of $L$ category descriptions $C=\{c_1,c_2,\cdots,c_L \}$, the goal is to learn a scoring function $g(x,c_i)$ that takes document $x$ and label description $c_i$ as input and produces a similarity score as the measure of how well the document and the label match to each other. 
%In the rest of the paper, we assume each input text as a sentence for convenience, which can be easily generalized to a multi-sentence passage or document without jeopardizing the key concepts.

In the zero-shot setting, text classification can be formulated as a sentence alignment problem, where both the both the input sentence and the label descriptions are encoded using a pre-trained sentence encoder like SimCSE~\cite{gao2021simcse}. The similarity scores between the sentence and labels embeddings are used to predict related labels. The performance can be further improved by converting a short label description into a full sentence via prompts~\cite{wang2023pesco, hong2022tess}. For example, the label ``sports" can be converted to ``This is an article about sports."
%Since this approach relies on the semantic matching between textual instances and label descriptions rather than the availability of labeled training data
%However, as label descriptions are often just a few words instead of long sentences, they may not provide enough context for a pre-trained encoder to grasp the semantic meaning of the labels. To address this issue, prompt-based approaches \cite{schick2020exploiting} convert label names into natural language sentences, namely \textit{label prompts}. For example, the label ``sports" can be converted to ``This is an article about sports." 
Following this, we denote by $p_i$ as the label prompt for a label description $c_i$, the scoring function can be implemented as:
\begin{equation}
    g(x, c_i)=\operatorname{sim}\left(f_\theta(x), f_\theta(p_i) \right)
\end{equation}
where $f_\theta(\cdot)$ is the sentence encoder parameterized by $\theta$ and $\mathrm{sim}(\cdot,\cdot)$ is a similarity function such as dot product or cosine similarity.

Given a input text at inference time, the predicted  label is the one with the highest similarity score:
\begin{equation}
\hat{y}=\argmax_j g\left(x, c_j\right) \label{eq:inference}
\end{equation}

\subsection{Self-Training with Contrastive Learning}
\label{subsec:self-training}
Self-training is an algorithm to enhance the generalization capability of models by learning from its own predictions~\cite{meng2020text,schick2021self,wang2023pesco}. 
%Specifically, it follows an iterative process where a pre-trained model is used to classify unlabeled data, and the newly classified data with high confidence is then used to further train the model. 
Since the predicted labels can be erroneous, studies have shown that soft labeling~\cite{xie2016unsupervised,meng2020text} or label smoothing~\cite{muller2019does} can prevent the model from becoming overly confident. In this work, we propose a loss function with soft labeling that connects supervised contrastive learning and entropy regularization~\cite{grandvalet2004semi}. Our analysis aims to reveal how self-training can improve the zero-shot generalization by maximizing the decision boundaries of ambiguous classes.

%We denote $f_\theta(x)$ as our sentence encoder model. 
Given a input text $x$, the predicted distribution of the label space is:
\begin{equation}
    P(\hat{y}_i | x ;\theta) =  \frac{\exp(\operatorname{sim}(f_\theta(x), f_\theta(p_i)))}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x), f_\theta(p_c)))} 
\end{equation}
Here, $p_i$ is a label prompt for label $c_i$. We define the target distribution as:
\begin{equation}
    Q(\hat{y}_i | x ;\theta) =   \frac{\exp(\operatorname{sim}(f_\theta(x), f_\theta(p_i))/\tau)}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x), f_\theta(p_c))/\tau)} \label{eq:soft-label}
\end{equation}
where $\tau \leq 1$ is the temperature. A lower temperature implies a sharper distribution and thus greater confidence in the predicted label. We drop the notation of $\theta$ for convenience.
The contrastive text to label ($t2l$) objective function is defined as:
\begin{equation}
    \mathcal{L}_{t2l} = -\sum_{i=1}^{N} \sum_{j=1}^{L} Q(\hat{y}_j|x_i)\log P(\hat{y}_j|x_i) \label{eq:loss}
\end{equation}
When $\tau \rightarrow 0$, $Q(\hat{y} | x)$ becomes categorical distribution and the loss reduces to a supervised contrastive learning loss with pseudo label $\hat{y}$ as the target:
\begin{equation}
    \mathcal{L}_{t2l}^{\tau \rightarrow 0} = -\sum_{i=1}^{N} \log P(\hat{y}|x_i)
\end{equation}
It encourages the model to predict label $\hat{y}$ given $x$ with more confident. 
On the other hand, when $\tau = 1$, the loss reduces to a minimization of conditional entropy function $H$:
\begin{align}
    &\mathcal{L}_{t2l}^{\tau = 1} = H\left(C \mid X \right) \\
    &= - \sum_{i=1}^N\sum_{j=1}^L P(\hat{y}_j|x_i)\log P(\hat{y}_j|x_i)
\end{align}
We show a theorem such that minimizing the loss function \eqref{eq:loss} can achieve similar effects Entropy Regularization~\cite{grandvalet2006entropy,grandvalet2004semi}, which is a means to enforce the cluster assumption such that the decision boundary should lie in low-density regions to improve generalization performance~\cite{chapelle2005semi}. 
\begin{theorem}
\label{theorem:paper}
Consider a binary classification problem with linearly separable labeled examples. When $0<\tau<1$, optimizing \eqref{eq:loss} with gradient descend will enforce the larger margin between classes and achieves max margin classifier under certain constraint. 
\end{theorem}
We place our formal theorems and proofs in Appendix \secref{sec:proofs}. Theorem \ref{theorem:1}  suggests that self-training is an in domain fine-tuning that maximizes class separation, which serves as an explanation why training on pseudo-labels can enhance performance even if no extra labeling information is provided.
In our experiment, we show empirically that self-training of smaller model can outperform Alpaca-7B prediction. We set $\tau = 0.1$ to balance supervised classification and low density separation between classes. 


%While self-learning was effective in improving the performance of our model, it is not without its limitations. One potential issue is overfitting to the pseudo label, which is prone to error. Additionally, self-learning requires a large amount of unlabeled data, which may not always be available.
%In the following section, we propose conditional augmentation methods with generative model in the training loop to make self-learning more robust. 

\label{subsec:conditional augment}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/fig_cond_aug.pdf}
    \caption{Augmented Text Generation Conditioned on Pseudo Labels: When a pseudo label is incorrect, it can mislead the training process and decrease classification performance. We generate augmented text conditioned on the pseudo label, aiming to make the generated text closer to the majority members in the category of the pseudo label. This approach aims to improve the quality of the generated instances for self-training. }
    \label{fig:conditional_aug_illustration}
\end{figure*}

\subsection{Input Text Augmentation}
\label{subsec:input augment}
In this section, we propose a way to enhance the semantic embedding of the original input text with multiple GPT-generated pieces of texts, as shown in \figref{fig:general_aug_illustration}. When the input text is relatively short, such as consisting of only one or a few sentences, the alignment-based matching to relevant labels may not be sufficiently effective. A natural remedy is to elaborate the input with a pre-trained GPT model to generate multiple pieces of texts. Specifically, we use a simple human instruction, "Elaborate the text with a few sentences," to guide the instruction-tuned GPT model, such as Alpaca-7B~\cite{alpaca}, in generating probable expansions and continuations of the text. Our system treats the concatenation of the input text and each GPT-generated piece as one augmentation, and then takes the average of the embeddings of multiple augmentations as the merged embedding of the augmented input. Intuitively, such an augmentation should enhance the semantic matching among input text and relevant labels if the meaning of the input is underrepresented (too short) and if the generative model is highly effective in generating relevant pieces for the given input.  The first assumption is often true in realist textual data, and the second condition is well-met by large pre-trained GPT models.  


Formally, the input text $x \sim P(x)$ can be viewed as randomly sampled from an underlying distribution, and the augmented texts can be viewed as the different variants sampled from the conditional probability distribution induced by the GPT model, denoted as $x^{\text{aug}} \sim P_g(\cdot | x)$. We obtain the augmented text embedding by averaging the embeddings of the multiple versions of the augmented text:
\begin{equation}
\frac{1}{K}\sum_{i=1}^K f_\theta(x \oplus x_i^{\text{aug}}),
\end{equation}
where $\oplus$ is the concatenation operator for text and $x_i^{\text{aug}}$ is the $i$-th sample from $P_g(\cdot | x)$. 
%Unlike previous work that generates multiple solutions for self-consistency by voting~\cite{wang2022self}, 
Our augmented texts provide different views of the input text, and the mean of the embedding provides an ensemble of induced features. We then use the augmented text embedding for pseudo-label prediction. If GPT is available at test time, we can use this method for inference as well.

\subsection{Augmentation Conditioned on Prediction}
% The success of the algorithm relies on two key factors: 1) the availability of diversified instances for self-training, and 2) the accurate assignment of pseudo label for the unlabeled text. However, it is difficult to satisfy the two conditions at the same time. On the one hand, if self-training is applied to only the highly confident instances, the amount of training instance is too limited to the effectiveness of the algorithm. On the other hand, if we apply the algorithm to large amount of unlabeled data with lower confidence, the inaccurate pseudo labeling can lead to negative transfer and hurt the performance of the classifier.
The loss function of \eqref{eq:loss} can effectively enhance the separability of class instances by enforcing the decision boundary to lie in low density regions of the embedding space. In each self-training iteration, when the sampled instances are labeled with relatively lower confidence, which lie near the decision boundary, the contrastive loss pushes the instances closer to the pseudo label prompt embedding. However, self-training can lead to an undesirable bias in the classifier when instances are mislabeled.
To address this issue, we propose a novel approach to the generation of labeled data for self-training.  That is, we use GPT to generate labeled training pairs by augmenting each input text conditioned on the system-predicted (pseudo) labels, as shown in \figref{fig:conditional_aug_illustration}. % which can be used to augment the original data and provide more accurate and diverse instances for self-training. 
For example, if a business news article discussing the retirement of Starbucks' president is misclassified with the label of "sports", optimizing the model with this mislabeled training instance will make the decision boundaries between business articles less separable from sport articles. To alleviate such an undesirable effect, we use GPT to augment the input text conditioned on the sport category, resulting in a text closer to the typical ones in the sport category instead of the original one which lies closely to the decision boundary between "sports" and "businesses". In other words, by using GPT to generate augmented texts conditioned on pseudo labels, we aim to enhance the system-produced training pair with better separation of class labels in the embedding space.  %as a sports article due to the presence of keywords like "sports," 
%optimizing on this mislabeled instance will push the business article further to sports category. 
%To alleviate this difficulty, we use GPT to expand the text from the sports aspect of the article, which looks like other true data points that belong to the sports category. 
%This approach can help prevent self-training from biasing the classifier and improve its overall performance. 

Based on the aforementioned intuition, we propose an approach called \textit{instruction-based conditional generation} to generate augmented text conditioned on the pseudo label. In this approach, we incorporate the predicted label information into the instructions provided to the model. For instance, we can use the instruction ``Discuss the sports aspects of the article" to guide the model in generating text that is more relevant to the sports category.

%By providing these instructions, we ensure the generated text is more accurate and diverse, which can alleviate the problem of overfitting to mislabeled data during self-training. In the following, w
Additionally, we propose two loss functions to enhance the self-training algorithm with the augmented text as follows.

\begin{algorithm*}[ht!]
  \caption{Self-training with GPT model assisted in the loop}
  \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, pre-trained GPT model $g(\cdot)$.\\
  \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
  \textbf{Input augmentation}: For each observed text, generate $K$ samples of augmented text from $P_g(\cdot | x)$.\\
  \For {$t: 1 \rightarrow T$ self-training iterations}
  {
    Use $f_{\theta}(\cdot)$ to generate pseudo-labels $\hat{y}$ (eq.\ref{eq:inference}) and soft-labels $Q$ (eq.\ref{eq:soft-label}) for texts with input augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ according to prediction confidence\;
    \For {each training sample $(x, \hat{y})$}
    {
        \eIf{key $(x, \hat{y}) \in \operatorname{GenDict}$}
        {
            Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
        }
        {
            Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}\;
            Add generated texts to $\operatorname{GenDict}$\Comment{Cached generated text}\;
        }
    }
    Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$.
  }
 % \textbf{Return:} $f_{\theta}(\cdot)$
\label{alg:self-train}
\end{algorithm*}

\subsubsection{Contrastive Learning for Conditionally Augmented Text and Label Prompt} To alleviate the problem of erroneous label assignment, we use the conditional augmented text ($x^{\text{c\_aug}} \sim P_g(\cdot | x, \hat{y})$) and the pseudo label prompt as positive pairs. 
\begin{equation}
    \mathcal{L}_{g2l} = -\sum_{i=1}^{N} \sum_{j=1}^{L} Q(\hat{y}_j|x_i^{\text{c\_aug}})\log P(\hat{y}_j|x_i^{\text{c\_aug}})
    %-\log P(\hat{y}_i | x ;\theta) = -\log \frac{\exp(\operatorname{sim}(f_\theta(x_\text{aug}), f_\theta(p_i)))}{\sum_{c\in C} \exp(\operatorname{sim}( f_\theta(x_\text{aug}), f_\theta(p_c)))} 
    \label{eq:g2l}
\end{equation}

\subsubsection{Contrastive Learning for Observed Text and Augmented Text} 
%The essence of contrastive learning is to compare different views of data for representation learning~\cite{chen2020simple,he2020momentum}. 
For document representation, the contrastive pairs are usually created by sampling spans of document~\cite{contriver}. In our case, the generative model naturally creates different views of data and we use the contrastive loss between observed text and generated text for optimization: 
\begin{equation} 
\begin{split}
     &\mathcal{L}_{t2g}=\sum_{i \in \mathit{I}} \frac{ -1}{|A(i)|} \\ 
     &\sum_{x^{\text{aug}} \in A(i)}\log{\frac{\exp({sim(f_{\theta}(x_i),f_{\theta}(x^{\text{aug}}) )})}{\sum_{j \in \mathit{I}}\exp(sim(f_{\theta}(x_i),f_{\theta}(x_j) ))}}.
\end{split} \label{eq:t2g}
\end{equation}
where $\mathit{I}$ is a training batch and $A(i)$ 
%\equiv  \{x^\prime_j , \forall j \in \mathit{I} :\hat{y}_j=\hat{y}_i\}$ 
denotes the set of augmented texts belonging to the same pseudo class of input $x_i$. 

\Algref{alg:self-train} shows the self-training of \ourmodel with generative model assisting in the self-training loop. During training, we found that a balanced sampling that keeps the same number ($S_t$ for iteration $t$) of training for each category is important for the stability of self-training. Additionally, we use a dictionary to cache the conditional generated text to avoid repeated generation. 




%Overall, our proposed approach provides a flexible and effective way to generate augmented text that can improve the performance of smaller classifiers. By conditioning the GPT model on the predicted label, we can generate additional text that is specifically tailored to the characteristics of each class, which can help the classifier better distinguish between different classes. Our approach can also help address the issues of limited diversity and inaccurate pseudo labeling in self-training, by providing more diverse and accurate instances for self-training.

%suffers from wrong labels. We condition the GPT model on the current predicted label to generate additional augmented text that is tailored to the specific label. We explore the following methods for conditional generation of augmented text $x^\prime \sim P_g(\cdot| x, \hat{y})$.

%In label-based conditional generation, we directly incorporate the predicted label $\hat{y}$ into the generation process. Specifically, we condition the GPT model on both the original text $x$ and the predicted label $\hat{y}$ to generate augmented text $x^\prime$. This approach allows the model to better capture the specific characteristics and features of each class.



% \subsubsection{Prompt-based Conditional Generation} To let the model condition on label, we append a short prompt after the original text $x$, such as ``In this sports article,". 

% \subsubsection{Instruction-based Conditional Generation}
% Previous work have shown that language models have the ability to take instructions~\cite{brown2020language,ouyang2022training}. We construction natural language instructions for the language model to generate augmented text, such as "continue writing the above paragraph from the perspective of sports".

% The GPT model can then generate additional text based on this prompt. By conditioning the model on the predicted label, we can generate augmented text that is specifically tailored to the characteristics of the sports class.

% Overall, these three methods provide flexible and effective ways to generate augmented text that can improve the performance of smaller classifiers. By conditioning the GPT model on the predicted label, we can generate additional text that is specifically tailored to the characteristics of each class, which can help the classifier better distinguish between different classes.

%\subsubsection{Generation with Word Mask} 
% Another approach for conditional generation is to give the model higher probability on topic sensitive words. In this paper, we propose a method based on topical words:
% \begin{align}
%     \delta &= p(w|y) - p(w|x) \\
%     p(w|x,y) &\propto \alpha(\delta)p(w|x)
% \end{align}
    
%~\cite{schick2021self} use 

% \begin{algorithm}
% $i\gets 10$\;
% \eIf{$i\geq 5$}
% {
%     $i\gets i-1$\;
% }{
%     \If{$i\leq 3$}
%     {
%         $i\gets i+2$\;
%     }
% }
% \end{algorithm}
  
% \begin{algorithm}
%   \caption{Self-training with GPT model in the training loop}
%   \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, pre-trained GPT model $g(\cdot)$.\\
%   \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
%   \begin{algorithmic}[1]
%   %\Procedure{Self-train}{$n$}
%   \State \textbf{General purpose augmentation}: For each observed text, sample $K$ views  from $P_g(\cdot | x)$ as general augmented data.
%   \For {$t: 1 \rightarrow T$ self-training iterations}:
%     \parState {Use $f_{\theta}(\cdot)$ to generate soft pseudo-labels $\hat{y}$ with eq.(\ref{eq:inference}) for unlabeled texts with general purpose augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ for each label according to confidence. }
%     \For {each training sample $(x, \hat{y})$}, 
%     \If{$(x, \hat{y}) \in \operatorname{GenDict}$}
%         \State Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
%     \Else
%         \State Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}
%         \State Add generated texts to $\operatorname{GenDict}$\Comment{cached generated text}
%     \EndIf
%     \EndFor
%     \parState {Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$ in eq~\ref{eq:loss}.}
%   \EndFor
    
%   \State \textbf{Return:} $f_{\theta}(\cdot)$
%   %\textbf{Final model:} Use $f_{\theta}(\cdot)$ to label the full unlabeled set, then uses the pseudo-labels to learn a new model as final model.
%   %\EndProcedure
%  \end{algorithmic}
%  \label{alg:self-train}
% \end{algorithm}

% \begin{algorithm}[ht!]
%   \caption{Self-training with GPT model in the training loop}
%   \textbf{Require:} Unlabeled texts $X$, label descriptions $C$, pre-trained GPT model $g(\cdot)$.\\
%   \textbf{Initialization:} Classifier $f_{\theta}(\cdot)$ initialized with pre-trained sentence encoder. Empty dictionary $\operatorname{GenDict}$ to cache conditional generated text.  \\
%   \textbf{General purpose augmentation}: For each observed text, sample $K$ views  from $P_g(\cdot | x)$ as general augmented data.\\
%   \For {$t: 1 \rightarrow T$ self-training iterations}
%   {
%     Use $f_{\theta}(\cdot)$ to generate soft pseudo-labels $\hat{y}$ with eq.(\ref{eq:inference}) for unlabeled texts with general purpose augmentation. Sample a balanced subset of pseudo-labeled training pairs of size $S_t$ for each label according to confidence\;
%     \For {each training sample $(x, \hat{y})$}
%     {
%         \eIf{$(x, \hat{y}) \in \operatorname{GenDict}$}
%         {
%             Fetch generated texts from $\operatorname{GenDict}$ \Comment{Use cached generated text}
%         }
%         {
%             Generate $M$ samples from $P_g(\cdot | x, \hat{y})$\Comment{Conditional augmentation}\;
%             Add generated texts to $\operatorname{GenDict}$\Comment{Cached generated text}\;
%         }
%     }
%     Use sampled training pairs and the conditionally generated text to update the parameters $\theta$ of $f_{\theta}(\cdot)$ with the objective function $\mathcal{L} = \mathcal{L}_{g2l} + \mathcal{L}_{t2g}$ in eq~\ref{eq:loss}.
%   }
%  % \textbf{Return:} $f_{\theta}(\cdot)$
% \label{alg:self-train}
% \end{algorithm}
